MaudeTypedLog: A Typed Interpreter for Prolog in Maude

Prolog is traditionally thought of as an untyped logic programming language, although there are queries that result in a type error. Several attempts of statically introducing a type discipline in Prolog have been made but they have not been widely adopted. We use Maude to implement a typed unification algorithm and use it as the basis for an interpreter for Prolog called MaudeTypedLog. This interpreter follows the Typed SLD-resolution operational semantics for logic programming, that makes it possible to detect type errors in both programs and queries dynamically.

==> eptcsdata.tex <==
\providecommand{\firstpage}{107}
\providecommand{\publicationstatus}{V. de Paiva; T.A. de Lima (Eds.): 21st International Symposium\\ on Logical and Semantic Frameworks, with Applications (LSFA 2026)\\
EPTCS 449, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.449.7}{10.4204/EPTCS.449.7}}
\pdfoutput=1

